Comparing restricted mean survival times in small sample clinical trials using pseudo-observations

The widely used proportional hazard assumption cannot be assessed reliably in small-scale clinical trials and might often in fact be unjustified, e.g. due to delayed treatment effects. An alternative to the hazard ratio as effect measure is the difference in restricted mean survival time (RMST) that does not rely on model assumptions. Although an asymptotic test for two-sample comparisons of the RMST exists, it has been shown to suffer from an inflated type I error rate in samples of small or moderate sizes. Recently, permutation tests, including the studentized permutation test, have been introduced to address this issue. In this paper, we propose two methods based on pseudo-observations (PO) regression models as alternatives for such scenarios and assess their properties in comparison to previously proposed approaches in an extensive simulation study. Furthermore, we apply the proposed PO methods to data from a clinical trail and, by doing so, point out some extension that might be very useful for practical applications such as covariate adjustments.

==> tables/tbl03-power.tex <==
\begin{table}

\caption{\label{tab:tbl-power}Rejection rates (power) of different methods in \% (nominal level $\alpha = 5\%$)}
\centering
\resizebox{\linewidth}{!}{
\begin{threeparttable}
\begin{tabular}[t]{l>{}c|ccc>{}c|ccc>{}c|cccc}
\toprule
\multicolumn{1}{c}{\textbf{ }} & \multicolumn{1}{c}{\textbf{ }} & \multicolumn{4}{c}{\textbf{$N = K \cdot (12, 18)$}} & \multicolumn{4}{c}{\textbf{$N = K \cdot (15, 15)$}} & \multicolumn{4}{c}{\textbf{$N = K \cdot (18, 12)$}} \\
\cmidrule(l{3pt}r{3pt}){3-6} \cmidrule(l{3pt}r{3pt}){7-10} \cmidrule(l{3pt}r{3pt}){11-14}
Censoring & K & Asy & Perm & PO1 & PO2 & Asy & Perm & PO1 & PO2 & Asy & Perm & PO1 & PO2\\
%\midrule
\addlinespace[0.5em]
\multicolumn{14}{l}{S1: Exponential distributions}\\
\hline
\hspace{1em}un. W. & 1 & <span style=" font-weight: bold;    " >25.1</span> & <span style="     " >18.5</span> & <span style="     " >20.4</span> & <span style="     " >17.7</span> & <span style=" font-weight: bold;    " >23.2</span> & <span style="     " >18.5</span> & <span style="     " >19.4</span> & <span style="     " >16.2</span> & <span style=" font-weight: bold;    " >23.0</span> & <span style="     " >17.8</span> & <span style="     " >18.0</span> & <span style="     " >12.0</span>\\
\hspace{1em} & 2 & <span style=" font-weight: bold;    " >35.9</span> & <span style="     " >32.4</span> & <span style="     " >33.5</span> & <span style="     " >32.7</span> & <span style=" font-weight: bold;    " >35.9</span> & <span style="     " >32.9</span> & <span style="     " >32.8</span> & <span style="     " >32.2</span> & <span style=" font-weight: bold;    " >34.0</span> & <span style="     " >30.8</span> & <span style="     " >31.2</span> & <span style="     " >29.8</span>\\
\hspace{1em} & 4 & <span style=" font-weight: bold;    " >60.9</span> & <span style="     " >59.0</span> & <span style="     " >59.5</span> & <span style="     " >59.6</span> & <span style=" font-weight: bold;    " >59.3</span> & <span style="     " >57.8</span> & <span style="     " >57.8</span> & <span style="     " >57.5</span> & <span style=" font-weight: bold;    " >57.0</span> & <span style="     " >55.2</span> & <span style="     " >55.1</span> & <span style="     " >54.7</span>\\
\hspace{1em} & 6 & <span style=" font-weight: bold;    " >77.7</span> & <span style="     " >76.8</span> & <span style="     " >76.9</span> & <span style="     " >76.9</span> & <span style=" font-weight: bold;    " >76.6</span> & <span style="     " >75.8</span> & <span style="     " >75.9</span> & <span style="     " >75.9</span> & <span style=" font-weight: bold;    " >74.0</span> & <span style="     " >72.8</span> & <span style="     " >72.7</span> & <span style="     " >72.5</span>\\
\cellcolor[HTML]{e9ecef}{\hspace{1em}eq. U.} & \cellcolor[HTML]{e9ecef}{1} & \cellcolor[HTML]{e9ecef}{<span style=" font-weight: bold;    " >24.1</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >18.8</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >20.2</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >17.5</span>} & \cellcolor[HTML]{e9ecef}{<span style=" font-weight: bold;    " >23.2</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >17.8</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >18.8</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >15.9</span>} & \cellcolor[HTML]{e9ecef}{<span style=" font-weight: bold;    " >23.3</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >17.2</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >18.7</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >13.6</span>}\\
\cellcolor[HTML]{e9ecef}{\hspace{1em}} & \cellcolor[HTML]{e9ecef}{2} & \cellcolor[HTML]{e9ecef}{<span style=" font-weight: bold;    " >35.1</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >32.2</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >32.4</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >31.7</span>} & \cellcolor[HTML]{e9ecef}{<span style=" font-weight: bold;    " >37.5</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >34.1</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >34.1</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >33.1</span>} & \cellcolor[HTML]{e9ecef}{<span style=" font-weight: bold;    " >36.2</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >32.2</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >32.8</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >31.6</span>}\\
\cellcolor[HTML]{e9ecef}{\hspace{1em}} & \cellcolor[HTML]{e9ecef}{4} & \cellcolor[HTML]{e9ecef}{<span style=" font-weight: bold;    " >61.9</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >60.2</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >60.4</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >60.4</span>} & \cellcolor[HTML]{e9ecef}{<span style=" font-weight: bold;    " >61.5</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >60.1</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >60.0</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >60.0</span>} & \cellcolor[HTML]{e9ecef}{<span style=" font-weight: bold;    " >59.4</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >57.6</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >57.9</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >57.3</span>}\\
\cellcolor[HTML]{e9ecef}{\hspace{1em}} & \cellcolor[HTML]{e9ecef}{6} & \cellcolor[HTML]{e9ecef}{<span style=" font-weight: bold;    " >76.5</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >75.7</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >75.7</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >75.7</span>} & \cellcolor[HTML]{e9ecef}{<span style=" font-weight: bold;    " >78.1</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >77.2</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >77.4</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >77.3</span>} & \cellcolor[HTML]{e9ecef}{<span style=" font-weight: bold;    " >75.6</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >74.8</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >74.7</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >74.7</span>}\\
\hspace{1em}eq. W. & 1 & <span style=" font-weight: bold;    " >24.8</span> & <span style="     " >20.0</span> & <span style="     " >21.1</span> & <span style="     " >19.0</span> & <span style=" font-weight: bold;    " >24.9</span> & <span style="     " >20.5</span> & <span style="     " >21.2</span> & <span style="     " >19.3</span> & <span style=" font-weight: bold;    " >24.9</span> & <span style="     " >19.6</span> & <span style="     " >20.8</span> & <span style="     " >17.5</span>\\
\hspace{1em} & 2 & <span style=" font-weight: bold;    " >39.7</span> & <span style="     " >36.5</span> & <span style="     " >37.0</span> & <span style="     " >36.2</span> & <span style=" font-weight: bold;    " >39.5</span> & <span style="     " >36.9</span> & <span style="     " >37.2</span> & <span style="     " >36.5</span> & <span style=" font-weight: bold;    " >37.6</span> & <span style="     " >34.6</span> & <span style="     " >35.0</span> & <span style="     " >34.0</span>\\
\hspace{1em} & 4 & <span style=" font-weight: bold;    " >64.5</span> & <span style="     " >63.1</span> & <span style="     " >63.2</span> & <span style="     " >62.9</span> & <span style=" font-weight: bold;    " >64.6</span> & <span style="     " >63.6</span> & <span style="     " >63.3</span> & <span style="     " >63.1</span> & <span style=" font-weight: bold;    " >64.1</span> & <span style="     " >62.8</span> & <span style="     " >62.8</span> & <span style="     " >62.6</span>\\
\hspace{1em} & 6 & <span style=" font-weight: bold;    " >81.4</span> & <span style="     " >80.6</span> & <span style="     " >80.7</span> & <span style="     " >80.7</span> & <span style=" font-weight: bold;    " >83.2</span> & <span style="     " >82.4</span> & <span style="     " >82.5</span> & <span style="     " >82.4</span> & <span style=" font-weight: bold;    " >79.2</span> & <span style="     " >78.2</span> & <span style="     " >78.4</span> & <span style="     " >78.4</span>\\
\hline
\addlinespace[0.5em]
\multicolumn{14}{l}{S7: Exponential and piecewise exponential distributions with crossing curves}\\
\hline
\hspace{1em}un. W. & 1 & <span style=" font-weight: bold;    " >21.4</span> & <span style="     " >15.5</span> & <span style="     " >17.7</span> & <span style="     " >15.2</span> & <span style=" font-weight: bold;    " >20.8</span> & <span style="     " >15.9</span> & <span style="     " >17.1</span> & <span style="     " >13.9</span> & <span style=" font-weight: bold;    " >20.7</span> & <span style="     " >16.2</span> & <span style="     " >17.1</span> & <span style="     " > 9.9</span>\\
\hspace{1em} & 2 & <span style=" font-weight: bold;    " >32.4</span> & <span style="     " >29.0</span> & <span style="     " >30.0</span> & <span style="     " >29.3</span> & <span style=" font-weight: bold;    " >31.6</span> & <span style="     " >28.6</span> & <span style="     " >29.0</span> & <span style="     " >28.2</span> & <span style=" font-weight: bold;    " >30.4</span> & <span style="     " >27.4</span> & <span style="     " >27.8</span> & <span style="     " >26.0</span>\\
\hspace{1em} & 4 & <span style=" font-weight: bold;    " >54.2</span> & <span style="     " >52.4</span> & <span style="     " >52.9</span> & <span style="     " >52.5</span> & <span style=" font-weight: bold;    " >52.7</span> & <span style="     " >51.1</span> & <span style="     " >50.8</span> & <span style="     " >50.7</span> & <span style=" font-weight: bold;    " >49.0</span> & <span style="     " >47.1</span> & <span style="     " >47.3</span> & <span style="     " >46.6</span>\\
\hspace{1em} & 6 & <span style=" font-weight: bold;    " >71.1</span> & <span style="     " >70.1</span> & <span style="     " >70.3</span> & <span style="     " >70.2</span> & <span style=" font-weight: bold;    " >69.2</span> & <span style="     " >68.2</span> & <span style="     " >68.4</span> & <span style="     " >68.1</span> & <span style=" font-weight: bold;    " >65.7</span> & <span style="     " >64.9</span> & <span style="     " >65.0</span> & <span style="     " >64.6</span>\\
\cellcolor[HTML]{e9ecef}{\hspace{1em}eq. U.} & \cellcolor[HTML]{e9ecef}{1} & \cellcolor[HTML]{e9ecef}{<span style=" font-weight: bold;    " >21.1</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >16.0</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >17.7</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >14.8</span>} & \cellcolor[HTML]{e9ecef}{<span style=" font-weight: bold;    " >21.1</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >16.3</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >17.7</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >14.5</span>} & \cellcolor[HTML]{e9ecef}{<span style=" font-weight: bold;    " >20.2</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >15.2</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >16.5</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " > 9.5</span>}\\
\cellcolor[HTML]{e9ecef}{\hspace{1em}} & \cellcolor[HTML]{e9ecef}{2} & \cellcolor[HTML]{e9ecef}{<span style=" font-weight: bold;    " >33.0</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >29.6</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >30.0</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >29.0</span>} & \cellcolor[HTML]{e9ecef}{<span style=" font-weight: bold;    " >32.1</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >29.6</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >30.0</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >29.1</span>} & \cellcolor[HTML]{e9ecef}{<span style=" font-weight: bold;    " >30.0</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >26.3</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >27.2</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >25.8</span>}\\
\cellcolor[HTML]{e9ecef}{\hspace{1em}} & \cellcolor[HTML]{e9ecef}{4} & \cellcolor[HTML]{e9ecef}{<span style=" font-weight: bold;    " >53.8</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >52.5</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >52.4</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >52.2</span>} & \cellcolor[HTML]{e9ecef}{<span style=" font-weight: bold;    " >53.5</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >52.0</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >52.3</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >51.8</span>} & \cellcolor[HTML]{e9ecef}{<span style=" font-weight: bold;    " >52.0</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >50.0</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >50.4</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >49.8</span>}\\
\cellcolor[HTML]{e9ecef}{\hspace{1em}} & \cellcolor[HTML]{e9ecef}{6} & \cellcolor[HTML]{e9ecef}{<span style=" font-weight: bold;    " >70.1</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >69.0</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >69.3</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >69.4</span>} & \cellcolor[HTML]{e9ecef}{<span style=" font-weight: bold;    " >70.2</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >69.0</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >69.2</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >69.2</span>} & \cellcolor[HTML]{e9ecef}{<span style=" font-weight: bold;    " >67.1</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >65.9</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >65.9</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >65.9</span>}\\
\hspace{1em}eq. W. & 1 & <span style=" font-weight: bold;    " >21.8</span> & <span style="     " >16.7</span> & <span style="     " >18.0</span> & <span style="     " >15.9</span> & <span style=" font-weight: bold;    " >21.5</span> & <span style="     " >17.4</span> & <span style="     " >18.3</span> & <span style="     " >15.6</span> & <span style=" font-weight: bold;    " >20.5</span> & <span style="     " >16.0</span> & <span style="     " >16.9</span> & <span style="     " >10.5</span>\\
\hspace{1em} & 2 & <span style=" font-weight: bold;    " >34.1</span> & <span style="     " >31.3</span> & <span style="     " >31.5</span> & <span style="     " >30.8</span> & <span style=" font-weight: bold;    " >33.4</span> & <span style="     " >30.7</span> & <span style="     " >31.2</span> & <span style="     " >30.3</span> & <span style=" font-weight: bold;    " >31.1</span> & <span style="     " >28.0</span> & <span style="     " >28.3</span> & <span style="     " >26.7</span>\\
\hspace{1em} & 4 & <span style=" font-weight: bold;    " >57.2</span> & <span style="     " >56.0</span> & <span style="     " >56.1</span> & <span style="     " >55.8</span> & <span style=" font-weight: bold;    " >57.2</span> & <span style="     " >56.0</span> & <span style="     " >55.9</span> & <span style="     " >55.8</span> & <span style=" font-weight: bold;    " >52.9</span> & <span style="     " >51.2</span> & <span style="     " >51.6</span> & <span style="     " >51.0</span>\\
\hspace{1em} & 6 & <span style=" font-weight: bold;    " >73.9</span> & <span style="     " >73.2</span> & <span style="     " >73.3</span> & <span style="     " >73.3</span> & <span style=" font-weight: bold;    " >73.8</span> & <span style="     " >73.1</span> & <span style="     " >73.1</span> & <span style="     " >72.9</span> & <span style=" font-weight: bold;    " >69.9</span> & <span style="     " >68.7</span> & <span style="     " >69.1</span> & <span style="     " >68.7</span>\\
\hline
\addlinespace[0.5em]
\multicolumn{14}{l}{S8: Weibull distributions with crossing curves and shape alternatives}\\
\hline
\hspace{1em}un. W. & 1 & <span style=" font-weight: bold;    " >40.5</span> & <span style="     " >32.9</span> & <span style="     " >35.5</span> & <span style="     " >31.3</span> & <span style=" font-weight: bold;    " >42.6</span> & <span style="     " >36.4</span> & <span style="     " >37.2</span> & <span style="     " >31.6</span> & <span style=" font-weight: bold;    " >41.3</span> & <span style="     " >35.4</span> & <span style="     " >35.8</span> & <span style="     " >26.9</span>\\
\hspace{1em} & 2 & <span style=" font-weight: bold;    " >62.2</span> & <span style="     " >58.4</span> & <span style="     " >59.4</span> & <span style="     " >58.1</span> & <span style=" font-weight: bold;    " >62.3</span> & <span style="     " >59.6</span> & <span style="     " >60.1</span> & <span style="     " >57.9</span> & <span style=" font-weight: bold;    " >59.6</span> & <span style="     " >56.2</span> & <span style="     " >56.4</span> & <span style="     " >51.1</span>\\
\hspace{1em} & 4 & <span style=" font-weight: bold;    " >88.1</span> & <span style="     " >86.9</span> & <span style="     " >87.2</span> & <span style="     " >87.2</span> & <span style=" font-weight: bold;    " >86.7</span> & <span style="     " >85.7</span> & <span style="     " >85.9</span> & <span style="     " >85.2</span> & <span style=" font-weight: bold;    " >84.0</span> & <span style="     " >83.2</span> & <span style="     " >83.1</span> & <span style="     " >82.2</span>\\
\hspace{1em} & 6 & <span style=" font-weight: bold;    " >96.6</span> & <span style="     " >96.4</span> & <span style="     " >96.5</span> & <span style="     " >96.3</span> & <span style=" font-weight: bold;    " >96.5</span> & <span style="     " >96.4</span> & <span style="     " >96.3</span> & <span style="     " >96.2</span> & <span style=" font-weight: bold;    " >94.4</span> & <span style="     " >94.2</span> & <span style="     " >94.1</span> & <span style="     " >93.8</span>\\
\cellcolor[HTML]{e9ecef}{\hspace{1em}eq. U.} & \cellcolor[HTML]{e9ecef}{1} & \cellcolor[HTML]{e9ecef}{<span style=" font-weight: bold;    " >37.9</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >30.0</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >31.7</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >26.2</span>} & \cellcolor[HTML]{e9ecef}{<span style=" font-weight: bold;    " >39.8</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >33.0</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >34.2</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >28.7</span>} & \cellcolor[HTML]{e9ecef}{<span style=" font-weight: bold;    " >39.2</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >31.8</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >34.0</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >26.1</span>}\\
\cellcolor[HTML]{e9ecef}{\hspace{1em}} & \cellcolor[HTML]{e9ecef}{2} & \cellcolor[HTML]{e9ecef}{<span style=" font-weight: bold;    " >61.4</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >57.1</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >57.9</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >56.6</span>} & \cellcolor[HTML]{e9ecef}{<span style=" font-weight: bold;    " >61.8</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >58.1</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >58.6</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >57.0</span>} & \cellcolor[HTML]{e9ecef}{<span style=" font-weight: bold;    " >59.6</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >55.5</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >56.5</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >53.3</span>}\\
\cellcolor[HTML]{e9ecef}{\hspace{1em}} & \cellcolor[HTML]{e9ecef}{4} & \cellcolor[HTML]{e9ecef}{<span style=" font-weight: bold;    " >86.7</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >85.7</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >85.8</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >85.7</span>} & \cellcolor[HTML]{e9ecef}{<span style=" font-weight: bold;    " >87.4</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >86.4</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >86.6</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >86.4</span>} & \cellcolor[HTML]{e9ecef}{<span style=" font-weight: bold;    " >85.3</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >83.9</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >84.1</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >83.6</span>}\\
\cellcolor[HTML]{e9ecef}{\hspace{1em}} & \cellcolor[HTML]{e9ecef}{6} & \cellcolor[HTML]{e9ecef}{<span style=" font-weight: bold;    " >96.5</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >96.2</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >96.2</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >96.2</span>} & \cellcolor[HTML]{e9ecef}{<span style=" font-weight: bold;    " >96.5</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >96.3</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >96.3</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >96.3</span>} & \cellcolor[HTML]{e9ecef}{<span style=" font-weight: bold;    " >95.7</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >95.4</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >95.3</span>} & \cellcolor[HTML]{e9ecef}{<span style="     " >95.1</span>}\\
\hspace{1em}eq. W. & 1 & <span style=" font-weight: bold;    " >42.9</span> & <span style="     " >36.4</span> & <span style="     " >37.7</span> & <span style="     " >33.7</span> & <span style=" font-weight: bold;    " >44.3</span> & <span style="     " >38.3</span> & <span style="     " >39.0</span> & <span style="     " >35.3</span> & <span style=" font-weight: bold;    " >44.2</span> & <span style="     " >38.0</span> & <span style="     " >39.3</span> & <span style="     " >32.8</span>\\
\hspace{1em} & 2 & <span style=" font-weight: bold;    " >67.5</span> & <span style="     " >64.5</span> & <span style="     " >65.1</span> & <span style="     " >64.0</span> & <span style=" font-weight: bold;    " >68.1</span> & <span style="     " >65.4</span> & <span style="     " >65.7</span> & <span style="     " >64.8</span> & <span style=" font-weight: bold;    " >64.6</span> & <span style="     " >61.3</span> & <span style="     " >62.0</span> & <span style="     " >59.2</span>\\
\hspace{1em} & 4 & <span style=" font-weight: bold;    " >92.3</span> & <span style="     " >91.5</span> & <span style="     " >91.8</span> & <span style="     " >91.7</span> & <span style=" font-weight: bold;    " >91.9</span> & <span style="     " >91.4</span> & <span style="     " >91.5</span> & <span style="     " >91.3</span> & <span style=" font-weight: bold;    " >90.1</span> & <span style="     " >89.3</span> & <span style="     " >89.4</span> & <span style="     " >89.0</span>\\
\hspace{1em} & 6 & <span style=" font-weight: bold;    " >98.6</span> & <span style="     " >98.4</span> & <span style="     " >98.5</span> & <span style="     " >98.4</span> & <span style=" font-weight: bold;    " >98.0</span> & <span style=" font-weight: bold;    " >98.0</span> & <span style="     " >97.9</span> & <span style="     " >97.9</span> & <span style=" font-weight: bold;    " >97.4</span> & <span style="     " >97.2</span> & <span style="     " >97.3</span> & <span style="     " >97.1</span>\\
\bottomrule
\end{tabular}
\begin{tablenotes}
\item \textit{Note:} Largest value per scenario is printed bold.
\item \textit{Abbreviations:} Asy, asymptotic test; Perm, studentized permutation test; PO1, pseudo-observations asymptotic; PO2, pseudo-observations bootstrap; un. W., unequal Weibull censoring; eq. U., equal uniform censoring; eq. W., equal Weibull censoring.
\end{tablenotes}
\end{threeparttable}}
\end{table}

